Discretization error cancellation in electronic structure calculation: a quantitative study

It is often claimed that error cancellation plays an essential role in quantum chemistry and first-principle simulation for condensed matter physics and materials science. Indeed, while the energy of a large, or even medium-size, molecular system cannot be estimated numerically within chemical accuracy (typically 1 kcal/mol or 1 mHa), it is considered that the energy difference between two configurations of the same system can be computed in practice within the desired accuracy. The purpose of this paper is to provide a quantitative study of discretization error cancellation. The latter is the error component due to the fact that the model used in the calculation (e.g. Kohn-Sham LDA) must be discretized in a finite basis set to be solved by a computer. We first report comprehensive numerical simulations performed with Abinit on two simple chemical systems, the hydrogen molecule on the one hand, and a system consisting of two oxygen atoms and four hydrogen atoms on the other hand. We observe that errors on energy differences are indeed significantly smaller than errors on energies, but that these two quantities asymptotically converge at the same rate when the energy cut-off goes to infinity. We then analyze a simple one-dimensional periodic Schr\"odinger equation with Dirac potentials, for which analytic solutions are available. This allows us to explain the discretization error cancellation phenomenon on this test case with quantitative mathematical arguments.

==> biblio_tot.tex <==
% Encoding: UTF-8

@Article{Gonze2009,
  author   = {Gonze, X. and Amadon, B. and Anglade, P.-M. and Beuken, J.-M. and Bottin, F. and Boulanger, P. and Bruneval, F. and Caliste, D. and Caracas, R. and C{\^{o}}t{\'{e}}, M. and Deutsch, T. and Genovese, L. and Ghosez, Ph and Giantomassi, M. and Goedecker, S. and Hamann, D.R. and Hermet, P. and Jollet, F. and Jomard, G. and Leroux, S. and Mancini, M. and Mazevet, S. and Oliveira, M.J.T. and Onida, G. and Pouillon, Y. and Rangel, T. and Rignanese, G.-M. and Sangalli, D. and Shaltaf, R. and Torrent, M. and Verstraete, M.J. and Zerah, G. and Zwanziger, J.W.},
  title    = {{ABINIT: First-principles approach to material and nanosystem properties}},
  journal  = {Comput. Phys. Comm.},
  year     = {2009},
  volume   = {180},
  number   = {12},
  pages    = {2582--2615},
  month    = {dec},
  issn     = {00104655},
  abstract = {ABINIT [http://www.abinit.org] allows one to study, from first-principles, systems made of electrons and nuclei (e.g. periodic solids, molecules, nanostructures, etc.), on the basis of Density-Functional Theory (DFT) and Many-Body Perturbation Theory. Beyond the computation of the total energy, charge density and electronic structure of such systems, ABINIT also implements many dynamical, dielectric, thermodynamical, mechanical, or electronic properties, at different levels of approximation. The present paper provides an exhaustive account of the capabilities of ABINIT. It should be helpful to scientists that are not familiarized with ABINIT, as well as to already regular users. First, we give a broad overview of ABINIT, including the list of the capabilities and how to access them. Then, we present in more details the recent, advanced, developments of ABINIT, with adequate references to the underlying theory, as well as the relevant input variables, tests and, if available, ABINIT tutorials. Program summary: Program title: ABINIT. Catalogue identifier: AEEU{\_}v1{\_}0. Distribution format: tar.gz. Journal reference: Comput. Phys. Comm. Programming language: Fortran95, PERL scripts, Python scripts. Computer: All systems with a Fortran95 compiler. Operating system: All systems with a Fortran95 compiler. Has the code been vectorized or parallelized?: Sequential, or parallel with proven speed-up up to one thousand processors. RAM: Ranges from a few Mbytes to several hundred Gbytes, depending on the input file. Classification: 7.3, 7.8. External routines: (all optional) BigDFT [1], ETSF IO [2], libxc [3], NetCDF [4], MPI [5], Wannier90 [6]. Nature of problem: This package has the purpose of computing accurately material and nanostructure properties: electronic structure, bond lengths, bond angles, primitive cell size, cohesive energy, dielectric properties, vibrational properties, elastic properties, optical properties, magnetic properties, non-linear couplings, electronic and vibrational lifetimes, etc. Solution method: Software application based on Density-Functional Theory and Many-Body Perturbation Theory, pseudopotentials, with planewaves, Projector-Augmented Waves (PAW) or wavelets as basis functions. Running time: From less than one second for the simplest tests, to several weeks. The vast majority of the {\textgreater}600 provided tests run in less than 30 seconds. References: [1] http://inac.cea.fr/LSim/BigDFT.[2] http://etsf.eu/index.php?page=standardization.[3] http://www.tddft.org/programs/octopus/wiki/index.php/Libxc.[4] http://www.unidata.ucar.edu/software/netcdf.[5] http://en.wikipedia.org/wiki/MessagePassingInterface.[6] http://www.wannier.org. {\textcopyright} 2009 Elsevier B.V. All rights reserved.},
  doi      = {10.1016/j.cpc.2009.07.007},
  isbn     = {0010-4655},
  keywords = {Density-Functional Theory,Electronic structure,First-principles calculation,Many-Body Perturbation Theory},
  pmid     = {273011500017},
  url      = {http://linkinghub.elsevier.com/retrieve/pii/S0010465509002276},
}
@article{Gonze2002,
abstract = {The density functional theory (DFT) computation of electronic structure, total energy and other properties of materials, is a field in constant progress. In order to stay at the forefront of knowledge, a DFT software project can benefit enormously from widespread collaboration, if handled properly. Also, modern software engineering concepts can considerably ease its development. The ABINIT project relies upon these ideas: freedom of sources, reliability, portability, and self-documentation are emphasised, in the development of a sophisticated plane-wave pseudopotential code. We describe ABINITv3.0, distributed under the GNU General Public License. The list of ABINITv3.0 capabilities is presented, as well as the different software techniques that have been used until now: PERL scripts and CPP directives treat a unique set of FORTRAN90 source files to generate sequential (or parallel) object code for many different platforms; more than 200 automated tests secure existing capabilities; strict coding rules are followed; the documentation is extensive, including online help files, tutorials, and HTML-formatted sources. ?? 2002 Elsevier Science B.V. All rights reserved.},
author = {Gonze, X. and Beuken, J.-M. and Caracas, R. and Detraux, F. and Fuchs, M. and Rignanese, G.-M. and Sindic, L. and Verstraete, M. and Zerah, G. and Jollet, F. and Torrent, M. and Roy, A. and Mikami, M. and Ghosez, Ph and Raty, J.-Y. and Allan, D.C.},
doi = {10.1016/S0927-0256(02)00325-7},
isbn = {0927-0256},
issn = {09270256},
journal = {Comput. Mat. Sci.},
keywords = {Density functional theory,Electronic structure,Software engineering},
month = {nov},
number = {3},
pages = {478--492},
title = {{First-principles computation of material properties: the ABINIT software project}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0927025602003257},
volume = {25},
year = {2002}
}

@Article{JCP,
  author   = {Canc{\`{e}}s, Eric and Dusson, Genevi{\`{e}}ve and Maday, Yvon and Stamm, Benjamin and Vohral{\'{i}}k, Martin},
  title    = {{A perturbation-method-based post-processing for the planewave discretization of Kohn–Sham models}},
  journal  = {J. Comput. Phys.},
  year     = {2016},
  volume   = {307},
  pages    = {446--459},
  month    = {feb},
  issn     = {00219991},
  abstract = {In this article, we propose a post-processing of the planewave solution of the Kohn-Sham LDA model with pseudopotentials. This post-processing is based upon the fact that the exact solution can be interpreted as a perturbation of the approximate solution, allowing us to compute corrections for both the eigenfunctions and the eigenvalues of the problem in order to increase the accuracy. Indeed, this post-processing only requires the computation of the residual of the solution on a finer grid so that the additional computational cost is negligible compared to the initial cost of the planewave-based method needed to compute the approximate solution. Theoretical estimates certify an increased convergence rate in the asymptotic convergence range. Numerical results confirm the low computational cost of the post-processing and show that this procedure improves the energy accuracy of the solution even in the pre-asymptotic regime which comprises the target accuracy of practitioners.},
  doi      = {10.1016/j.jcp.2015.12.012},
  keywords = {Density-functional theory,Nonlinear eigenvalue problem,Perturbation method,Planewave approximation,Post-processing},
  url      = {http://linkinghub.elsevier.com/retrieve/pii/S002199911500830X},
}

@Article{Cances2014,
  author   = {Canc{\`{e}}s, {\'{E}}ric and Dusson, Genevi{\`{e}}ve and Maday, Yvon and Stamm, Benjamin and Vohral{\'{i}}k, Martin},
  title    = {{A perturbation-method-based a posteriori estimator for the planewave discretization of nonlinear Schr{\"{o}}dinger equations}},
  journal  = {C.R. Math.},
  year     = {2014},
  volume   = {352},
  number   = {11},
  pages    = {941--946},
  month    = {nov},
  issn     = {1631073X},
  abstract = {In this Note, we propose a new method, based on perturbation theory, to post-process the planewave approximation of the eigenmodes of periodic Schr??dinger operators. We then use this post-processing to construct an accurate a posteriori estimator for the approximations of the (nonlinear) Gross-Pitaevskii equation, valid at each step of a self-consistent procedure. This allows us to design an adaptive algorithm for solving the Gross-Pitaevskii equation, which automatically refines the discretization along the convergence of the iterative process, by means of adaptive stopping criteria. Dans cette Note, nous proposons une nouvelle m??thode, bas??e sur la th??orie des perturbations, pour post-traiter l'approximation dans une base d'ondes planes des modes propres d'op??rateurs de Schr??dinger p??riodiques. Nous utilisons ensuite ce post-traitement pour construire un estimateur d'erreur a posteriori pour les approximations de l'??quation de Gross-Pitaevskii (non lin??aire), valide ?? chaque ??tape de la proc??dure auto-coh??rente. Ceci nous permet de proposer un algorithme adaptatif pour r??soudre cette ??quation, qui raffine automatiquement la discr??tisation au cours du processus it??ratif, par le biais de crit??res d'arr??t adaptatifs.},
  doi      = {10.1016/j.crma.2014.09.014},
  url      = {http://linkinghub.elsevier.com/retrieve/pii/S1631073X1400212X},
}

@Article{Zhou2013,
  author   = {Chen, Huajie and Gong, Xingao and He, Lianhua and Yang, Zhang and Zhou, Aihui},
  title    = {{Numerical analysis of finite dimensional approximations of Kohn–Sham models}},
  journal  = {Adv. Comput. Math.},
  year     = {2013},
  volume   = {38},
  number   = {2},
  pages    = {225--256},
  month    = {feb},
  issn     = {1019-7168},
  abstract = {In this paper, we study finite dimensional approximations of Kohn--Sham models, which are widely used in electronic structure calculations. We prove the convergence of the finite dimensional approximations and derive the a priori error estimates for ground state energies and solutions. We also provide numerical simulations for several molecular systems that support our theory.},
  doi      = {10.1007/s10444-011-9235-y},
  isbn     = {1044401192},
  keywords = {Convergence,Density functional theory,Error estimate,Kohn-Sham equation,Nonlinear eigenvalue problem},
  url      = {http://link.springer.com/10.1007/s10444-011-9235-y},
}

@Article{Dusson2016,
  author   = {Dusson, Genevi{\`{e}}ve and Maday, Yvon},
  title    = {{A posteriori analysis of a nonlinear Gross–Pitaevskii-type eigenvalue problem}},
  journal  = {IMA J. Numer. Anal.},
  year     = {2016},
  pages    = {drw001},
  month    = {may},
  issn     = {0272-4979},
  doi      = {10.1093/imanum/drw001},
  keywords = {a posteriori analysis,approximation,iterative solution algorithm,nonlinear eigenvalue problem,plane wave,stopping criteria},
  url      = {http://imajna.oxfordjournals.org/cgi/doi/10.1093/imanum/drw001},
}

@Article{Goedecker1996,
  author        = {Goedecker, S. and Teter, M. and Hutter, J.},
  title         = {{Separable dual-space Gaussian pseudopotentials}},
  journal       = {Phys. Rev. B},
  year          = {1996},
  volume        = {54},
  number        = {3},
  pages         = {1703--1710},
  month         = {jul},
  issn          = {0163-1829},
  abstract      = {We present pseudopotential coefficients for the first two rows of the Periodic Table. The pseudopotential is of an analytic form that gives optimal efficiency in numerical calculations using plane waves as a basis set. At most, seven coefficients are necessary to specify its analytic form. It is separable and has optimal decay properties in both real and Fourier space. Because of this property, the application of the nonlocal part of the pseudopotential to a wave function can be done efficiently on a grid in real space. Real space integration is much faster for large systems than ordinary multiplication in Fourier space, since it shows only quadratic scaling with respect to the size of the system. We systematically verify the high accuracy of these pseudopotentials by extensive atomic and molecular test calculations. {\textcopyright} 1996 The American Physical Society.},
  doi           = {10.1103/PhysRevB.54.1703},
  isbn          = {1098-0121},
  pmid          = {9986014},
  url           = {http://link.aps.org/doi/10.1103/PhysRevB.54.1703{\%}5Cnhttp://arxiv.org/abs/mtrl-th/9512004 http://link.aps.org/doi/10.1103/PhysRevB.54.1703},
}

@Article{Kohn1965,
  author        = {Kohn, W. and Sham, L. J.},
  title         = {{Self-Consistent Equations Including Exchange and Correlation Effects}},
  journal       = {Phys. Rev. },
  year          = {1965},
  volume        = {140},
  number        = {4A},
  pages         = {A1133--A1138},
  month         = {nov},
  issn          = {0031-899X},
  abstract      = {From a theory of Hohenberg and Kohn, approximation methods for treating an inhomogeneous system of interacting electrons are developed. These methods are exact for systems of slowly varying or high density. For the ground state, they lead to self-consistent equations analogous to the Hartree and Hartree-Fock equations, respectively. In these equations the exchange and correlation portions of the chemical potential of a uniform electron gas appear as additional effective potentials. (The exchange portion of our effective potential differs from that due to Slater by a factor of -';.) Electronic systems at finite temperatures and in magnetic lelds are also treated by similar methods. An appendix deals with a further correction for systems with short-wavelength density oscillations.},
  doi           = {10.1103/PhysRev.140.A1133},
  isbn          = {9783540373674},
  pmid          = {20432011},
  primaryclass  = {10.1103},
  url           = {http://link.aps.org/doi/10.1103/PhysRev.140.A1133},
}
@article{Chen15,
author = {Chen, Huajie and Schneider, Reinhold},
doi = {10.1051/m2an/2014052},
issn = {0764-583X},
journal = {ESAIM: Math. Model. and Num. Anal.},
month = {may},
number = {3},
pages = {755--785},
title = {{Numerical analysis of augmented plane wave methods for full-potential electronic structure calculations}},
url = {http://dx.doi.org/10.1051/m2an/2014052 http://www.esaim-m2an.org/10.1051/m2an/2014052},
volume = {49},
year = {2015}
}

@Article{Gygi95,
  author    = {Gygi, Fran{\c{c}}ois and Galli, Giulia},
  title     = {{Real-space adaptive-coordinate electronic-structure calculations}},
  journal   = {Phys. Rev. B},
  year      = {1995},
  volume    = {52},
  number    = {4},
  pages     = {R2229--R2232},
  month     = {jul},
  issn      = {0163-1829},
  doi       = {10.1103/PhysRevB.52.R2229},
  publisher = {American Physical Society},
  url       = {http://link.aps.org/doi/10.1103/PhysRevB.52.R2229},
}
@book{Helgaker,
address = {Chichester, UK},
author = {Helgaker, Trygve and J{\o}rgensen, Poul and Olsen, Jeppe},
doi = {10.1002/9781119019572},
isbn = {9781119019572},
keywords = {imported},
month = {aug},
publisher = {John Wiley {\&} Sons, Ltd},
title = {{Molecular Electronic-Structure Theory}},
url = {http://doi.wiley.com/10.1002/9781119019572},
year = {2000}
}
@inproceedings{Li11,
address = {New York, New York, USA},
author = {Li, Sheng and Chen, Ke and Hsieh, Ming-Yu and Muralimanohar, Naveen and Kersey, Chad D and Brockman, Jay B and Rodrigues, Arun F and Jouppi, Norman P},
booktitle = {Proceedings of 2011 International Conference for High Performance Computing, Networking, Storage and Analysis on - SC '11},
doi = {10.1145/2063384.2063445},
isbn = {9781450307710},
issn = {2167-4329},
keywords = {BCH,Checkpointing,DRAM,ECC,ECC scheme,Error analysis,Error correction codes,Exascale computing,Memory management,Program processors,Random access memory,Reliability,SECDED,checkpointing,chipkill,error correction codes,exascale computing,exascale system,fault tolerance,fault tolerant computing,hardware-related failure,memory errors,memory reliability,memory system,memory-intensive application,multiprocessing systems,reliability,storage management,system energy-delay product,system resiliency,tagged memory,tagged memory system},
month = {nov},
pages = {1},
publisher = {ACM Press},
title = {{System implications of memory reliability in exascale computing}},
url = {http://dl.acm.org/citation.cfm?doid=2063384.2063445},
year = {2011}
}

@Article{Gavini13,
  author    = {Motamarri, P and Nowak, M.R. and Leiter, K and Knap, J and Gavini, V},
  title     = {{Higher-order adaptive finite-element methods for Kohn–Sham density functional theory}},
  journal   = {J. Comput. Phys.},
  year      = {2013},
  volume    = {253},
  pages     = {308--343},
  month     = {nov},
  issn      = {00219991},
  doi       = {10.1016/j.jcp.2013.06.042},
  keywords  = {Computational efficiency,Convergence,Density functional theory,Finite elements,H-p refinement,Higher-order,Mesh adaption,Real space,Scalability,Spectral elements},
  publisher = {Academic Press Inc.},
  url       = {http://linkinghub.elsevier.com/retrieve/pii/S0021999113004774},
}

@book{ReedSimon1,
address = {New York},
author = {Reed, Michael and Simon, Barry},
isbn = {0-12-585050-6},
number = {6},
publisher = {Academic Press Inc.},
title = {{Methods of Modern Mathematical Physics. I. Functional Analysis}},
volume = {53},
year = {1972}
}

@Article{Cances2010,
  author   = {Canc{\`{e}}s, Eric and Chakir, Rachida and Maday, Yvon},
  title    = {{Numerical Analysis of Nonlinear Eigenvalue Problems}},
  journal  = {J. Sci. Comput.},
  year     = {2010},
  volume   = {45},
  number   = {1-3},
  pages    = {90--117},
  month    = {oct},
  issn     = {0885-7474},
  abstract = {We provide a priori error estimates for variational approximations of the ground state energy, eigenvalue and eigenvector of nonlinear elliptic eigenvalue problems of the form −div(A ∇ u)+Vu+f(u 2)u={\$}\lambda{\$} u, {\{}{\$}{\}}{\{}\backslash{\}}|u{\{}\backslash{\}}|{\{}{\_}{\}}{\{}{\{}{\}}L{\^{}}{\{}{\{}{\}}2{\{}{\}}{\}}{\{}{\}}{\}}=1{\{}{\$}{\}} . We focus in particular on the Fourier spectral approximation (for periodic problems) and on the ℙ1 and ℙ2 finite-element discretizations. Denoting by (u {\$}\delta{\$} ,{\$}\lambda{\$} {\$}\delta{\$} ) a variational approximation of the ground state eigenpair (u,{\$}\lambda{\$}), we are interested in the convergence rates of {\{}{\$}{\}}{\{}\backslash{\}}|u{\{}{\_}{\}}{\{}{\{}{\}}{\{}\backslash{\}}delta{\{}{\}}{\}}-u{\{}\backslash{\}}|{\{}{\_}{\}}{\{}{\{}{\}}H{\^{}}{\{}{\{}{\}}1{\{}{\}}{\}}{\{}{\}}{\}}{\{}{\$}{\}} , {\{}{\$}{\}}{\{}\backslash{\}}|u{\{}{\_}{\}}{\{}{\{}{\}}{\{}\backslash{\}}delta{\{}{\}}{\}}-u{\{}\backslash{\}}|{\{}{\_}{\}}{\{}{\{}{\}}L{\^{}}{\{}{\{}{\}}2{\{}{\}}{\}}{\{}{\}}{\}}{\{}{\$}{\}} , |{\$}\lambda{\$} {\$}\delta{\$} −{\$}\lambda{\$}|, and the ground state energy, when the discretization parameter {\$}\delta{\$} goes to zero. We prove in particular that if A, V and f satisfy certain conditions, |{\$}\lambda{\$} {\$}\delta{\$} −{\$}\lambda{\$}| goes to zero as {\{}{\$}{\}}{\{}\backslash{\}}|u{\{}{\_}{\}}{\{}{\{}{\}}{\{}\backslash{\}}delta{\{}{\}}{\}}-u{\{}\backslash{\}}|{\{}{\_}{\}}{\{}{\{}{\}}H{\^{}}{\{}{\{}{\}}1{\{}{\}}{\}}{\{}{\}}{\}}{\^{}}{\{}{\{}{\}}2{\{}{\}}{\}}+{\{}\backslash{\}}|u{\{}{\_}{\}}{\{}{\{}{\}}{\{}\backslash{\}}delta{\{}{\}}{\}}-u{\{}\backslash{\}}|{\{}{\_}{\}}{\{}{\{}{\}}L{\^{}}{\{}{\{}{\}}2{\{}{\}}{\}}{\{}{\}}{\}}{\{}{\$}{\}} . We also show that under more restrictive assumptions on A, V and f, |{\$}\lambda{\$} {\$}\delta{\$} −{\$}\lambda{\$}| converges to zero as {\{}{\$}{\}}{\{}\backslash{\}}|u{\{}{\_}{\}}{\{}{\{}{\}}{\{}\backslash{\}}delta{\{}{\}}{\}}-u{\{}\backslash{\}}|{\{}{\_}{\}}{\{}{\{}{\}}H{\^{}}{\{}{\{}{\}}1{\{}{\}}{\}}{\{}{\}}{\}}{\^{}}{\{}{\{}{\}}2{\{}{\}}{\}}{\{}{\$}{\}} , thus recovering a standard result for linear elliptic eigenvalue problems. For the latter analysis, we make use of estimates of the error u {\$}\delta{\$} −u in negative Sobolev norms.},
  doi      = {10.1007/s10915-010-9358-1},
  url      = {http://dx.doi.org/10.1007/s10915-010-9358-1 http://link.springer.com/10.1007/s10915-010-9358-1},
}
@article{M2AN12,
author = {Canc{\`{e}}s, Eric and Chakir, Rachida and Maday, Yvon},
doi = {10.1051/m2an/2011038},
issn = {0764-583X},
journal = {ESAIM: Math. Model. and Num. Anal.},
month = {mar},
number = {2},
pages = {341--388},
title = {{Numerical analysis of the planewave discretization of some orbital-free and Kohn-Sham models}},
url = {http://www.esaim-m2an.org/10.1051/m2an/2011038},
volume = {46},
year = {2012}
}
@article{Chen14,
author = {Chen, Huajie and Dai, Xiaoying and Gong, Xingao and He, Lianhua and Zhou, Aihui},
doi = {10.1137/130916096},
issn = {1540-3459},
journal = {Multiscale Model. {\&} Sim.},
month = {jan},
number = {4},
pages = {1828--1869},
title = {{Adaptive Finite Element Approximations for Kohn--Sham Models}},
url = {http://dx.doi.org/10.1137/130916096 http://epubs.siam.org/doi/abs/10.1137/130916096},
volume = {12},
year = {2014}
}

@Article{chen2015,
  author    = {Chen, Huajie and Schneider, Reinhold},
  title     = {{Error Estimates of Some Numerical Atomic Orbitals in Molecular Simulations}},
  journal   = {Comm. Comput. Phys.},
  year      = {2015},
  volume    = {18},
  number    = {01},
  pages     = {125--146},
  month     = {jul},
  issn      = {1815-2406},
  abstract  = {Numerical atomic orbitals have been successfully used in molecular simulations as a basis set, which provides a nature, physical description of the electronic states and is suitable for ?( N ) calculations based on the strictly localized property. This paper presents a numerical analysis for some simplified atomic orbitals, with polynomial-type and confined Hydrogen-like radial basis functions respectively. We give some a priori error estimates to understand why numerical atomic orbitals are computationally efficient in electronic structure calculations.},
  address   = {Cambridge, UK},
  doi       = {10.4208/cicp.170414.231214a},
  publisher = {Cambridge University Press},
  url       = {https://www.cambridge.org/core/article/div-class-title-error-estimates-of-some-numerical-atomic-orbitals-in-molecular-simulations-div/900E7103DDF7408411C93F4EE567EDE7 http://www.journals.cambridge.org/abstract{\_}S1815240615000523},
}

@Article{QuantumEspresso,
  author   = {Giannozzi, Paolo and Baroni, Stefano and Bonini, Nicola and Calandra, Matteo and Car, Roberto and Cavazzoni, Carlo and Ceresoli, Davide and Chiarotti, Guido L and Cococcioni, Matteo and Dabo, Ismaila and {Dal Corso}, Andrea and de Gironcoli, Stefano and Fabris, Stefano and Fratesi, Guido and Gebauer, Ralph and Gerstmann, Uwe and Gougoussis, Christos and Kokalj, Anton and Lazzeri, Michele and Martin-Samos, Layla and Marzari, Nicola and Mauri, Francesco and Mazzarello, Riccardo and Paolini, Stefano and Pasquarello, Alfredo and Paulatto, Lorenzo and Sbraccia, Carlo and Scandolo, Sandro and Sclauzero, Gabriele and Seitsonen, Ari P and Smogunov, Alexander and Umari, Paolo and Wentzcovitch, Renata M},
  title    = {{QUANTUM ESPRESSO: a modular and open-source software project for quantum simulations of materials}},
  journal  = {J. Phys.: Condens. Matter},
  year     = {2009},
  volume   = {21},
  number   = {39},
  pages    = {395502},
  month    = {sep},
  issn     = {0953-8984},
  abstract = {QUANTUM ESPRESSO is an integrated suite of computer codes for electronic-structure calculations and materials modeling, based on density-functional theory, plane waves, and pseudopotentials (norm-conserving, ultrasoft, and projector-augmented wave). The acronym ESPRESSO stands for opEn Source Package for Research in Electronic Structure, Simulation, and Optimization . It is freely available to researchers around the world under the terms of the GNU General Public License. QUANTUM ESPRESSO builds upon newly-restructured electronic-structure codes that have been developed and tested by some of the original authors of novel electronic-structure algorithms and applied in the last twenty years by some of the leading materials modeling groups worldwide. Innovation and efficiency are still its main focus, with special attention paid to massively parallel architectures, and a great effort being devoted to user friendliness. QUANTUM ESPRESSO is evolving towards a distribution of independent and interoperable codes in the spirit of an open-source project, where researchers active in the field of electronic-structure calculations are encouraged to participate in the project by contributing their own codes or by implementing their own ideas into existing codes.},
  doi      = {10.1088/0953-8984/21/39/395502},
  url      = {http://stacks.iop.org/0953-8984/21/i=39/a=395502 http://stacks.iop.org/0953-8984/21/i=39/a=395502?key=crossref.c21336c286fa6d3db893262ae3f6e151},
}
@article{Lin15,
author = {Kaye, Jason and Lin, Lin and Yang, Chao},
doi = {10.4310/CMS.2015.v13.n7.a5},
issn = {15396746},
journal = {Comm. in Math. Sci.},
number = {7},
pages = {1741--1773},
title = {{{\textless}i{\textgreater}A posteriori{\textless}/i{\textgreater} error estimator for adaptive local basis functions to solve Kohn–Sham density functional theory}},
url = {http://www.intlpress.com/site/pub/pages/journals/items/cms/content/vols/0013/0007/a005/},
volume = {13},
year = {2015}
}

@Article{VASP,
  author    = {Kresse, G and Furthm{\"{u}}ller, J},
  title     = {{Efficient iterative schemes for ab initio total-energy calculations using a plane-wave basis set}},
  journal   = {Phys. Rev. B},
  year      = {1996},
  volume    = {54},
  number    = {16},
  pages     = {11169--11186},
  month     = {oct},
  issn      = {0163-1829},
  doi       = {10.1103/PhysRevB.54.11169},
  publisher = {American Physical Society},
  url       = {http://link.aps.org/doi/10.1103/PhysRevB.54.11169},
}

@Article{Kutzelnigg,
  author  = {Kutzelnigg, Werner},
  title   = {{Rate of convergence of basis expansions in quantum chemistry}},
  journal = {AIP Conf. Proc.},
  year    = {2012},
  volume  = {1504},
  number  = {1},
  pages   = {15--30},
  doi     = {10.1063/1.4771700},
  url     = {http://aip.scitation.org/doi/abs/10.1063/1.4771700 http://scitation.aip.org/content/aip/proceeding/aipcp/10.1063/1.4771700},
}
@article{BigDFT,
author = {Mohr, Stephan and Ratcliff, Laura E and Boulanger, Paul and Genovese, Luigi and Caliste, Damien and Deutsch, Thierry and Goedecker, Stefan},
doi = {10.1063/1.4871876},
issn = {0021-9606},
journal = {J. of Chem. Phys.},
month = {may},
number = {20},
pages = {204110},
title = {{Daubechies wavelets for linear scaling density functional theory}},
url = {http://aip.scitation.org/doi/abs/10.1063/1.4871876 http://aip.scitation.org/doi/10.1063/1.4871876},
volume = {140},
year = {2014}
}

@Article{Pask05,
  author   = {Pask, J E and Sterne, P A},
  title    = {{Finite element methods in ab initio electronic structure calculations}},
  journal  = {Modell. Simul. Mater. Sci. Eng.},
  year     = {2005},
  volume   = {13},
  number   = {3},
  pages    = {R71--R96},
  month    = {apr},
  issn     = {0965-0393},
  abstract = {We review the application of the finite element (FE) method to ab initio electronic structure calculations in solids. The FE method is a general approach for the solution of differential and integral equations which uses a strictly local, piecewise-polynomial basis. Because the basis is composed of polynomials, the method is completely general and its accuracy is systematically improvable. Because the basis is strictly local in real space, the method allows for variable resolution in real space; produces sparse, structured matrices, enabling the effective use of iterative solution methods; and is well suited for parallel implementation. The method thus combines significant advantages of both real-space-grid and basis-oriented approaches, and so is well suited for large, accurate ab initio calculations. We review the construction and properties of the required FE bases and their use in the self-consistent solution of the Kohn–Sham equations of density functional theory.},
  doi      = {10.1088/0965-0393/13/3/R01},
  url      = {http://stacks.iop.org/0965-0393/13/i=3/a=R01 http://stacks.iop.org/0965-0393/13/i=3/a=R01?key=crossref.fd888dfaf8db7901a4ea72e79c414dad},
}

@Article{Saad10,
  author  = {Saad, Yousef and Chelikowsky, James R and Shontz, Suzanne M},
  title   = {{Numerical Methods for Electronic Structure Calculations of Materials}},
  journal = {SIAM Rev.},
  year    = {2010},
  volume  = {52},
  number  = {1},
  pages   = {3--54},
  month   = {jan},
  issn    = {0036-1445},
  doi     = {10.1137/060651653},
  url     = {http://dx.doi.org/10.1137/060651653 http://epubs.siam.org/doi/abs/10.1137/060651653},
}

@Article{Maday2003,
  author   = {Maday, Y. and Turinici, G.},
  title    = {{Error bars and quadratically convergent methods for the numerical simulation of the Hartree-Fock equations}},
  journal  = {Numer. Math.},
  year     = {2003},
  volume   = {94},
  number   = {4},
  pages    = {739--770},
  issn     = {0029-599X},
  abstract = {Summary. This paper presents an a posteriori error analysis of the discretization methods used in computational quantum chemistry on the Hartree-Fock equations. Upper and lower bounds for the energy are obtained from any discrete approximation strategy of the solution and the estimator proposed is shown to possess further approximation virtues.},
  doi      = {10.1007/s002110100358},
  keywords = {Mathematics and Statistics},
  url      = {http://hal.upmc.fr/docs/00/79/83/21/PDF/R01020.pdf},
}


@article{Lin2016,
abstract = {{\textcopyright} 2016 EDP Sciences, SMAI.We present the first systematic work for deriving a posteriori error estimates for general non-polynomial basis functions in an interior penalty discontinuous Galerkin (DG) formulation for solving second order linear PDEs. Our residual type upper and lower bound error estimates measure the error in the energy norm. The main merit of our method is that the method is parameter-free, in the sense that all but one solution-dependent constants appearing in the upper and lower bound estimates are explicitly computable by solving local eigenvalue problems, and the only non-computable constant can be reasonably approximated by a computable one without affecting the overall effectiveness of the estimates in practice. As a side product of our formulation, the penalty parameter in the interior penalty formulation can be automatically determined as well. We develop an efficient numerical procedure to compute the error estimators. Numerical results for a variety of problems in 1D and 2D demonstrate that both the upper bound and lower bound are effective.},
author = {Lin, Lin and Stamm, Benjamin},
doi = {10.1051/m2an/2015069},
issn = {0764-583X},
journal = {ESAIM: Math. Model. and Num. Anal.},
keywords = {Discontinuous Gale,[A posteriori error estimation},
month = {jul},
number = {4},
pages = {1193--1222},
title = {{A posteriori error estimates for discontinuous Galerkin methods using non-polynomial basis functions Part I: Second order linear PDE}},
url = {http://www.esaim-m2an.org/10.1051/m2an/2015069},
volume = {50},
year = {2016}
}



@Article{Hanrath2008,
  author    = {Hanrath, Michael},
  title     = {{Wavefunction quality and error estimation of single- and multi-reference coupled-cluster and CI methods: The {\textless}mml:math altimg="si21.gif" display="inline" overflow="scroll" xmlns:xocs="http://www.elsevier.com/xml/xocs/dtd" xmlns:xs="http://www.w3.org/2001/}},
  journal   = {Chem. Phys. Lett.},
  year      = {2008},
  volume    = {466},
  number    = {4-6},
  pages     = {240--246},
  month     = {dec},
  issn      = {00092614},
  abstract  = {Different diagnostics for the approximation quality of wavefunction methods are discussed: the weighted T1 and D1 norm, the deviation from the full configuration interaction wavefunction, and the variance of the trial wavefunction. All diagnostics are evaluated for the H4 model system. Various wavefunction based approaches are analyzed. The wavefunction variance performs as a very reliable quantity to estimate the accuracy of the wavefunction and the energy expectation value. Although significantly more expensive than the evaluation of a plain energy expectation value the calculation of the wavefunction variance seems to be a comprehensive substitute for a full configuration interaction calculation. ?? 2008 Elsevier B.V. All rights reserved.},
  doi       = {10.1016/j.cplett.2008.10.046},
  isbn      = {0009-2614},
  publisher = {Elsevier B.V.},
  url       = {http://dx.doi.org/10.1016/j.cplett.2008.10.046 http://linkinghub.elsevier.com/retrieve/pii/S0009261408014176},
}

@Article{Kutzelnigg1991,
  author   = {Kutzelnigg, Werner},
  title    = {{Error analysis and improvements of coupled-cluster theory}},
  journal  = {Theor. Chim. Acta},
  year     = {1991},
  volume   = {80},
  number   = {4-5},
  pages    = {349--386},
  issn     = {0040-5744},
  abstract = {Summary. The in the energy of the traditional - (TCC) approach and of several variants is analyzed in terms of the 6 of the cluster operator S. A key feature of this is that TCC can be based on an energy functional (asymmetric in S and S*) that is made},
  doi      = {10.1007/BF01117418},
  isbn     = {1432-2234},
  keywords = {Coupled-cluster (CC) theory,Coupled-pair functional (CPF),Quadratic CI (QCI),Variational CC-Unitary CC},
  url      = {http://link.springer.com/10.1007/BF01117418},
}

@Article{Pernot2015,
  author   = {Pernot, Pascal and Civalleri, Bartolomeo and Presti, Davide and Savin, Andreas},
  title    = {{Prediction Uncertainty of Density Functional Approximations for Properties of Crystals with Cubic Symmetry}},
  journal  = {J. Phys. Chem. A},
  year     = {2015},
  volume   = {119},
  number   = {21},
  pages    = {5288--5304},
  month    = {may},
  issn     = {1089-5639},
  abstract = {The performance of a method is generally measured by an assessment of the errors between the method's results and a set of reference data. The prediction uncertainty is a measure of the confidence that can be attached to a method's prediction. Its estimation is based on the random part of the errors which cannot be explained by reference data uncertainty, which implies an evaluation of the systematic component(s) of the errors. As the predictions of most density functional approximations (DFA) present systematic errors, the standard performance statistics such as the mean of the absolute errors (MAE or MUE), cannot be directly used to infer prediction uncertainty. We investigate here an a posteriori calibration method to estimate the prediction uncertainty of DFAs for properties of solids. A linear model is shown to be adequate to address the systematic trend in the errors. The applicability of this approach to modest-size reference sets (28 systems) is evaluated for the prediction of band gaps, bulk moduli and lattice constants with a wide panel of DFAs.},
  doi      = {10.1021/jp509980w},
  pmid     = {25626469},
  url      = {http://pubs.acs.org/doi/abs/10.1021/jp509980w},
}

@Article{Pieniazek2008,
  author   = {Pieniazek, Susan N. and Clemente, Fernando R. and Houk, Kendall N.},
  title    = {{Sources of Error in DFT Computations of CC Bond Formation Thermochemistries: $\pi$→$\sigma$ Transformations and Error Cancellation by DFT Methods}},
  journal  = {Angew. Chem. Int. Ed.},
  year     = {2008},
  volume   = {47},
  number   = {40},
  pages    = {7746--7749},
  month    = {sep},
  issn     = {14337851},
  abstract = {No Abstract},
  doi      = {10.1002/anie.200801843},
  isbn     = {1433-7851},
  keywords = {Addition reactions,Computational chemistry,Density functional calculations,Hydrocarbons,Thermochemistry},
  pmid     = {18752237},
  url      = {http://doi.wiley.com/10.1002/anie.200801843},
}
@article{Rohwedder2013,
author = {Rohwedder, Thorsten and Schneider, Reinhold},
doi = {10.1051/m2an/2013075},
issn = {0764-583X},
journal = {ESAIM: Math. Model. and Num. Anal.},
keywords = {and phrases,coupled cluster method,electronic schr,error estimators,linear operator equation,non-,numerical analysis,odinger equation,quantum chemistry,quasi-optimality},
month = {nov},
number = {6},
pages = {1553--1582},
title = {{Error estimates for the Coupled Cluster method}},
url = {http://dx.doi.org/10.1051/m2an/2013075 http://www.esaim-m2an.org/10.1051/m2an/2013075},
volume = {47},
year = {2013}
}

